A Hybrid Approach to Secure Function Evaluation Using SGX

A protocol for two-party secure function evaluation (2P-SFE) aims to allow the parties to learn the output of function $f$ of their private inputs, while leaking nothing more. In a sense, such a protocol realizes a trusted oracle that computes $f$ and returns the result to both parties. There have been tremendous strides in efficiency over the past ten years, yet 2P-SFE protocols remain impractical for most real-time, online computations, particularly on modestly provisioned devices. Intel's Software Guard Extensions (SGX) provides hardware-protected execution environments, called enclaves, that may be viewed as trusted computation oracles. While SGX provides native CPU speed for secure computation, previous side-channel and micro-architecture attacks have demonstrated how security guarantees of enclaves can be compromised. In this paper, we explore a balanced approach to 2P-SFE on SGX-enabled processors by constructing a protocol for evaluating $f$ relative to a partitioning of $f$. This approach alleviates the burden of trust on the enclave by allowing the protocol designer to choose which components should be evaluated within the enclave, and which via standard cryptographic techniques. We describe SGX-enabled SFE protocols (modeling the enclave as an oracle), and formalize the strongest-possible notion of 2P-SFE for our setting. We prove our protocol meets this notion when properly realized. We implement the protocol and apply it to two practical problems: privacy-preserving queries to a database, and a version of Dijkstra's algorithm for privacy-preserving navigation. Our evaluation shows that our SGX-enabled SFE scheme enjoys a 38x increase in performance over garbled-circuit-based SFE. Finally, we justify modeling of the enclave as an oracle by implementing protections against known side-channels.

==> onlyabs.tex <==
  A protocol for two-party secure function evaluation (2P-SFE) aims to allow the
  parties to learn the output of function~$f$ of their private inputs, while
  leaking nothing more.
  In a sense, such a protocol realizes a trusted oracle that computes~$f$ and
  returns the result to both parties.
  There have been tremendous strides in efficiency over the past ten years, yet
  2P-SFE protocols remain impractical for most real-time, online computations,
  particularly on modestly provisioned devices.

  Intel's Software Guard Extensions (SGX) provides for hardware-protected
  execution environments, called \emph{enclaves}, that may be viewed
  as trusted computation oracles.
  However, this trust is somewhat misplaced, since these devices expose side-channels in practice.
  We explore a balanced approach to 2P-SFE on SGX-enabled processors
  through constructing
  a protocol for evaluating~$f$ \emph{relative to a partitioning of~$f$.}
  This approach alleviates the burden of trust on the enclave by allowing the
  protocol designer to choose which components should be evaluated within the
  enclave, and which via standard cryptographic techniques.

  We describe SGX-enabled SFE protocols (modeling the enclave as an oracle),
  and formalize the strongest-possible notion of 2P-SFE for our setting. We
  prove our protocol meets this notion, when properly realized.
  We implement the protocol and apply it to two practical problems:
  privacy-preserving queries to a database, and a version of Dijkstra's
  algorithm for privacy-preserving navigation.  Our evaluation shows
  that our SGX-enabled SFE scheme enjoys a 38x increase in performance over
  garbled-circuit-based SFE.
  Finally, we justify modeling of the enclave as an oracle by implementing
  protections against known side-channels.

